Spoof detection using time-delay shallow neural network and feature switching

Detecting spoofed utterances is a fundamental problem in voice-based biometrics. Spoofing can be performed either by logical accesses like speech synthesis, voice conversion or by physical accesses such as replaying the pre-recorded utterance. Inspired by the state-of-the-art \emph{x}-vector based speaker verification approach, this paper proposes a time-delay shallow neural network (TD-SNN) for spoof detection for both logical and physical access. The novelty of the proposed TD-SNN system vis-a-vis conventional DNN systems is that it can handle variable length utterances during testing. Performance of the proposed TD-SNN systems and the baseline Gaussian mixture models (GMMs) is analyzed on the ASV-spoof-2019 dataset. The performance of the systems is measured in terms of the minimum normalized tandem detection cost function (min-t-DCF). When studied with individual features, the TD-SNN system consistently outperforms the GMM system for physical access. For logical access, GMM surpasses TD-SNN systems for certain individual features. When combined with the decision-level feature switching (DLFS) paradigm, the best TD-SNN system outperforms the best baseline GMM system on evaluation data with a relative improvement of 48.03\% and 49.47\% for both logical and physical access, respectively.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> performanceAnalysisTab.tex <==
\section{Front-end features}
\label{sec:featureDescription}
In the recent literature related to ASV-spoof-2015 and ASV-spoof-2017 challenges, numerous works have been proposed with the focus on the feature extraction module~\cite{asv_spoof_2015_featuresUsed,IS2018_dlfs_replayAttacks}. The best feature is expected to capture the spectral variations among the spoofed and bonafide trials. Most of these works use a simple GMM classifier at the back-end. Initially, like many neural network system, spectrogram of the utterances were given as the input to the \emph{x}-vector architecture. However, the performance of the system with spectrogram input is worse. Hence, in this work, a set of features were chosen to build a spoof detection system with both GMM and \emph{x}-vector classifier. 

Constant-Q cepstral coefficients (CQCC) proposed in~\cite{cqcc} is known to be a robust feature in detecting the logical attacks. Linear frequency cepstral coefficients (LFCC) is shown to have better performance in case of the reverberant speech~\cite{lfcc_mfcc_comparison}. CQCC and LFCC features are given as the baseline features for ASV-spoof-2019 challenge. Along with CQCC and LFCC, we explore two other cepstral features namely Mel frequency cepstral coefficients (MFCC) and inverse Mel frequency cepstral coefficients (IMFCC). Inferences in ASV-spoof-2017 showed that the cepstral features are too coarse to detect the imperceptible spectral differences in the spoofed utterances~\cite{IS2018_dlfs_replayAttacks}. Hence, along with these cepstral coefficients, we also explore the effects of filterbank energies as features. Three filterbank energies namely linear frequency filterbank energy (LFBE), Mel frequency filterbank energy (MFBE) and Inverse Mel frequency filterbank energy (IMFBE) were chosen for the purpose. 



\begin{table*}
    \centering
    \setlength\extrarowheight{2pt}
    \begin{tabular}{c|c|c||c|c|c|c|c|c|c|c|c|c}
    \hline
         & \multirow{2}{*}{\bf System} & \multirow{2}{*}{\bf Metric} & \bf Overall  &  \multicolumn{8}{c}{\bf Type of physical attack conditions} \\ \cline{5-13}
         &  & & \bf Performance & AA & AB & AC & BA & BB & BC & CA & CB & CC \\ \cline{2-13}
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell{Baseline}}}  & \multirow{2}{*}{CQCC} & EER & 11.04 & 25.28 & 6.16 & 2.13 & 21.87 & 5.26  & 1.61 & 21.10 & 4.70 & 1.79 \\
         &  & t-DCF & 0.25 & 0.50 & 0.18 & 0.05 & 0.47 & 0.15 & 0.05 & 0.50 & 0.14 & 0.05 \\ \cline{3-13}
         & \multirow{2}{*}{LFCC} & EER & 13.54 & 32.48 & 4.40 & 3.95 & 24.59 & 4.29 & 3.20 & 21.63 & 3.92 & 3.06 \\
         &  & t-DCF & 0.30 & 0.74 & 0.13 & 0.11 & 0.60 & 0.13 & 0.09 & 0.55 & 0.12 & 0.09 \\ \hline
         \multirow{8}{*}{\rotatebox[origin=c]{90}{\makecell{Submitted}}}  & \multirow{2}{*}{Primary} & EER & 11.28 & 27.57 & 7.86 & 3.50 & 20.48 & 6.36 & 2.78 & 18.44 & 5.74 & 3.07 \\
         &  & t-DCF & 0.28 & 0.52 & 0.22 & 0.09 & 0.46 & 0.19 & 0.08 & 0.46 & 0.17 & 0.09 \\ \cline{3-13}
         & \multirow{2}{*}{Contrastive-1} & EER & 9.33 & 23.94 & 4.42 & 2.60 & 18.98 & 4.19 & 2.25 & 16.12 & 4.09 & 2.34 \\
         &  & t-DCF & 0.23 & 0.48 & 0.13 & 0.07 & 0.42 & 0.13 & 0.06 & 0.40 & 0.13 & 0.07 \\ \cline{3-13}
         & \multirow{2}{*}{Contrastive-2} & EER & 11.34 & 27.39 & 8.71 & 4.22 & 19.96 & 7.53 & 3.43 & 17.88 & 6.86 & 3.58  \\
         &  & t-DCF & 0.31 & 0.54 & 0.26 & 0.11 & 0.47 & 0.23 & 0.09 & 0.46 & 0.21 &0.10  \\ \cline{3-13}
         & \multirow{2}{*}{Single} & EER & 12.10 & 17.87 & 8.88 & 5.76 & 19.53 & 9.56 & 5.93 & 21.87 & 10.33 & 6.60 \\
         &  & t-DCF & 0.31 & 0.42 & 0.25 & 0.16 & 0.48 & 0.28 & 0.17 & 0.51 & 0.30 & 0.19 \\ \hline
    \end{tabular}
    \caption{Performance details of physical attacks based on the attack conditions}
    \label{tab:evalResults_PA_analysis}
\end{table*}


\begin{table*}[h]
    \begin{minipage}{\textwidth}
        \begin{minipage}[b]{0.6\textwidth}
            \centering
            \includegraphics[width=0.9\textwidth]{Figures/softfocal.pdf}
	        \captionof{figure}{The architecture of the \emph{x}-vector model for spoof detection.}
	        \label{fig:focal}
        \end{minipage}
        \hfill
        \begin{minipage}[b]{0.4\textwidth}
            \captionsetup{type=table} 
            \centering
            \setlength\extrarowheight{2pt}
            \resizebox{0.95\linewidth}{!}{
            \begin{tabular}{c|c|c|c|c}
                \hline
                \multirow{2}{*}{Type} & \multirow{2}{*}{System} & \multirow{2}{*}{Features} & \multicolumn{2}{c}{System Name} \\ \cline{4-5}
                & & & GMM & x-Vector \\ \hline
                \multirow{6}{*}{Single} & \multirow{6}{*}{Baseline} & CQCC & G-CQCC & x-CQCC  \\
                & & LFCC & G-LFCC & x-LFCC \\
                & & IMFCC & G-IMFCC & x-IMFCC \\
                & & LFBE & G-LFBE & x-LFBE \\  \hline
                \multirow{3}{*}{\makecell{DLFS}} & Primary & CQCC+LFBE & G-Prim & x-Prim \\ \cline{2-5}
                & Contrastive-1 & CQCC+LFCC & G-C1 & x-C1 \\  \cline{2-5}
                & Contrastive-2 & CQCC+LFBE & G-C2 & x-C2 \\ \hline
            \end{tabular}
            }
            \label{tab:systemsDeveloped}
        \end{minipage}
  \end{minipage}
\end{table*}
